The Spectral Distribution of Random Graphs with Given Degree Sequences

In this article, we study random graphs with a given degree sequence $d_1, d_2, \cdots, d_n$ from the configuration model. We show that under mild assumptions of the degree sequence, the spectral distribution of the normalized Laplacian matrix of such random graph converges in distribution to the semicircle distribution as the number of vertices $n\rightarrow \infty$. This extends work by McKay (1981) and Tran, Vu and Wang (2013) which studied random regular graphs ($d_1=d_2=\cdots=d_n=d$). Furthermore, we extend the assumption to show that a slightly more general condition is equivalent to the weak convergence to semicircle distribution. The equivalence is also illustrated by numerical simulations.

==> unused_proofs.tex <==
\begin{proof}
The sketch of our proof is very simple: since the proportion of the degrees less than $C\sqrt{\frac{D}{n}}$ is asymptotically going to $0$, we drop this proportion of the degrees and show that the effect of this dropping action is very small. In other words, the pruned graph, where all degrees are now larger than $C\sqrt{\frac{D}{n}}$, will still have $n(1 - o(1))$ vertices. Then, we can safely apply the results from Theorem \ref{semicircle} to the pruned graph and conclude that the eigenvalue distribution converges weakly to the semicircle law. 

In this proof, we rely on a previous paper \cite{JL07} about graph pruning. In this paper, the authors also investigate the configuration model under arbitrary degree sequences. They prune the graph by eliminating all vertices with degrees less than $k$ and draw conclusions about the number of vertices and edges in the remaining graph. For the conciseness of notation, we call those vertices with degrees larger than $k$ as heavy vertices and other vertices as light vertices. Note that the difficulty of this task lies in the fact that the action of eliminating light vertices will also eliminate a fraction of half-edges connected to heavy vertices and make them light vertices. We want to make sure that this pruning process will not go on forever and lead to an empty set of vertices in the remaining graph. 

Before introducing their main theorem, a few notations are necessary. We use $W$ to denote the empirical degree distribution $\p (W = r) = p_r $ where $p_r$ is the proportion of vertices with degree $r$. Then we consider a thinning $W_p$ of $W$, where we first sample an integer $r$ from the distribution of $W$ and then sample a Binomial distribution with parameters $r$ and $0<p<1$. We use $\pi_{lr}(p) = \p (\text{Bin}(l,p) = r) = $${l}\choose{r}$$p^r(1-p)^{l-r}$ to denote the Binomial probabilities. We use $\lambda = \frac{D}{n}$ to denote the average degree.

\begin{theorem}[Theorem 2.3 in \cite{JL07}]
Consider the random multigraph $G^*(n, (d_i)^n)$ for a sequence $(d_i)^n$. Let $k \geq 2$ be fixed, and let $\text{Core}^*_k$ be the $k$-core of $G^*(n, (d_i)^n)$. Let $\hat{p}$ be the largest $p \leq 1$ such that $\lambda p^2 = \E[W_{p} \mathbbm{1} [W_{p} \geq k]]$.

If $\hat{p} > 0$, and further $\lambda p^2 < h(p)$ for $p$ in some interval $(\hat{p} - \varepsilon, \hat{p})$, then whp $\text{Core}^*_k$ is non-empty, and $v(\text{Core}^*_k)/n \rightarrow \p(W_{\hat{p}} \geq k)$, $e(\text{Core}^*_k)/n \rightarrow \E[W_{\hat{p}} \mathbbm{1} [W_{\hat{p}} \geq k]]/2 = \lambda \hat{p}^2/2$.

\end{theorem}

We will not directly use the conclusion of this theorem. However, the techniques used in proving this theorem will be significant and relevant in obtaining Theorem \ref{equiv}. Below we start to discuss the two important techniques in \cite{JL07} that will help us finish our proof.

The first important technique is how we model the graph pruning process. We view the vertices as bins and half-edges as balls in the bins. Similarly, we call heavy vertices as heavy bins and light vertices as light bins. Therefore, the pruning procedure is the same as removing balls in pairs of two, one from the light bin and one from a random bin, until there are no light bins. Alternatively, we may change the order a bit, by first removing a random light ball and then start removing balls in pairs of two, one from a random bin and one from a light bin. Secondly, we introduce the concept of colors. We color all the balls white in the beginning and remove one random light ball. Subsequently, instead of removing balls in pairs of two, we remove one ball from a random bin and color a random white ball from a light bin red until there are no white balls available in any light bins. Therefore, if we consider only the white balls, this is the same process as before. Finally, we make this process in continuous time such that when there are $n$ balls available at time $t$, we wait for the amount of time of exponential distribution with parameter $n$ before the operation on the next pair of balls. Equivalently, we conduct an exponential process at rate $n$. The advantage of it is that each ball will be deleted at a rate $1$. We use $L(t)$ and $H(t)$ to denote the number of light bins and heavy balls at time $t$. We use $H_1(t)$ to denote the number of heavy bins at time $t$. We use $\tau$ to denote the stopping time when there are no white balls in the light bins. Such modeling techniques allow for the use of the Glivenko-Cantelli Theorem and are important in proving the main theorem in \cite{JL07}.

The second important part is the quantity $\hat{p}$ as a solution to $\lambda p^2 = \E[W_{p} \mathbbm{1} [W_{p} \geq k]]$. It is related to the concentration of the stopping time $\tau$. Suppose $\tau$ will concetrate to $\hat{t}$. Then we have the relationship $\hat{p} = e^{-\hat{t}}$ or $\hat{t} = - \log \hat{p}$. In other words, the continuous-time exponential process, as defined previously, will stop at time $\hat{t}$ with high probability. The detailed argument is in 

Now let us circle back to our setting. Firstly, we need to find out the order of $\hat{t}$. This is done by solving the equation
\begin{align*}
    &\lambda p^2 = \E[W_{p} \mathbbm{1} [W_{p} \geq k]] \\
    \Rightarrow & \lambda e^{-2t} = \E[W_{e^{-t}} \mathbbm{1} [W_{e^{-t}} \geq k]] \\
    \Rightarrow & \lambda e^{-2t} = \sum_{i: d_i e^{-t} > C \sqrt{\frac{D}{n}}} \frac{1}{n} d_i e^{-t} \\
    \Rightarrow & \frac{D}{n} e^{-t} = \sum_{i: d_i e^{-t} > C \sqrt{\frac{D}{n}}} \frac{1}{n} d_i \\
    \Rightarrow & t = - \log (\frac{ \sum_{i: d_i e^{-t} > C \sqrt{\frac{D}{n}}} d_i }{D} ) \\
    \Rightarrow & t = - \log (\frac{ \sum_{i: d_i > C \sqrt{\frac{D}{n}}} d_i }{D} )
\end{align*}
The last line is because we can see that $t$ will go to $0$ asymptotically and thus $e^{-t}$ will go to $1$ asymptotically. Therefore, we know that the rough order of $\hat{t}$ is $- \log (\frac{ \sum_{i: d_i > C \sqrt{\frac{D}{n}}} d_i }{D} )$. 

The quantity of $\hat{t}$ means that if we run this exponential process, we will ensure that no light vertices exist at time $\hat{t}$. Therefore, all we need to do is simply count the number of heavy vertices left in the remaining graph, without worrying that the deleted vertices will further transform heavy vertices into light vertices.

% Since this expression might not be intuitive enough to see its magnitude, we also derive below an upper bound of it with a more explicit manitude

Secondly, we consider the exponential process defined previously. Since each half-edge has a rate of $1$ to be deleted, the expected number of half-edges deleted at time $t$ will be $P = n(1-e^{-\hat{t}}) = \frac{n \sum_{i: d_i < C \sqrt{\frac{D}{n}}} d_i}{D} \leq \frac{n}{D} \epsilon n C\sqrt{\frac{D}{n}} = \epsilon C \frac{n^{\frac{3}{2}}}{D^{\frac{1}{2}}}$. Now we divide the heavy vertices into two groups. The first group contains vertices with degrees between $C\sqrt{\frac{D}{n}}$ and $2C\sqrt{\frac{D}{n}}$. The second group contains vertices with degrees between $2C\sqrt{\frac{D}{n}}$ and $n$. Note that in order for each vertex in the second group to become a light vertex, at least $C\sqrt{\frac{D}{n}}$ copies of half-edges must be deleted. Now, in order to give a conservative upper bound of the number of vertices deleted, we evenly distribute such $P$ copies of half-edges to vertices in the second group and assume that each vertex is assigned $C\sqrt{\frac{D}{n}}$ copes and gets deleted. Therefore, the number of vertices deleted in the second group, in this extreme case, is atmost
\begin{align*}
    \frac{P}{C\sqrt{\frac{D}{n}}} = \frac{\epsilon C \frac{n^{\frac{3}{2}}}{D^{\frac{1}{2}}}}{C\sqrt{\frac{D}{n}}} = \frac{\epsilon n^2}{D} = \frac{\epsilon n}{\lambda}
\end{align*}
where we know that the number of vertices being deleted in the second group cannot exceed the above quantity with probability $1$. 

However, this is the case when the stopping time $\tau$ exactly concentrates on its expectation $\hat{t}$. There may be fluctuations around the concentration. According to Lemma 4.2 and Lemma 4.3 in \cite{JL07}, which used Glivenko-Cantelli theorem, as well as an exact rate on the Glivenko-Cantelli theorem in \cite{Ma90}, we know that 
$$\p (|t - \hat{t}| > \epsilon' ) \leq 2 e^{-n\epsilon'^2}$$
This extra fluctuation may lead to a loss of additional $n \epsilon'$ half-edges. Again, if we evenly distribute such half-edges among vertices in the second group and assume that each vertex gets deleted after receiving $C\sqrt{\frac{D}{n}}$, the additional number of vertives deleted is atmost
\begin{align*}
    \frac{n\epsilon'}{C\sqrt{\frac{D}{n}}} =  \frac{\epsilon' n^{\frac{3}{2}}}{C D^{\frac{1}{2}}} = \frac{\epsilon' n}{C\sqrt{\lambda}}
\end{align*}

Therefore, let us summarize the work we have done so far. When the exponential process stops, we want to count the number vertices whose degrees are still greater than $C\sqrt{\frac{D}{n}}$ and thus remain in the pruned graph. Our goal is to show that the number of vertices after pruning will be almost the same as the original number of vertices. In this procedure, we're being conservative in the sense that we deleted more vertices than the process did and thus obtained an lower bound of the number of vertices in the remaining graph. Firstly, we abandon the proportion of vertices in the first group, whose degrees are smaller than $2C\sqrt{\frac{D}{n}}$. In this step we drop atmost $\epsilon n$ vertices. Note that the number is $\epsilon n $ because we can simiply let $C = 2C$ and choose a larger $n$ to make the proportion of vertices less than $2C\sqrt{\frac{D}{n}}$ equal $\epsilon$. Secondly, we abandon the vertices in the second group, because of the expected number of half-edges deleted. In this step we drop $\frac{\epsilon n }{\lambda}$. Thirdly, we abandon the vertices in the second group, because of the fluctuations around the expected number of half-edges delted. In this step we drop at most $\frac{\epsilon' n}{C\sqrt{\lambda}}$ with probability $2 e^{-n\epsilon'^2}$. Suppose $U_n$ is the number of vertices in the pruned graph. In general, we achieve the following non-asymptotic statement
$$\p (U_n < n - \epsilon n - \frac{\epsilon n}{\lambda} - \frac{\epsilon' n}{C\sqrt{\lambda}} ) \leq 2 e^{-n\epsilon'^2}$$

Therefore, after graph pruning, the number of vertices left will be $n (1 - o(1)) $ with high probability. We can thus apply the proof of moments method to the pruned graph and show that, in probability, the empirical eigenvalue distribution will converge to the semicircle distribution weakly. 

\end{proof}

